Large Language Models for Education: A Survey and Outlook

The advent of Large Language Models (LLMs) has brought in a new era of possibilities in the realm of education. This survey paper summarizes the various technologies of LLMs in educational settings from multifaceted perspectives, encompassing student and teacher assistance, adaptive learning, and commercial tools. We systematically review the technological advancements in each perspective, organize related datasets and benchmarks, and identify the risks and challenges associated with deploying LLMs in education. Furthermore, we outline future research opportunities, highlighting the potential promising directions. Our survey aims to provide a comprehensive technological picture for educators, researchers, and policymakers to harness the power of LLMs to revolutionize educational practices and foster a more effective personalized learning environment.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

==> draft.tex <==
% @inproceedings{chan2019recurrent,
%   title={A recurrent BERT-based model for question generation},
%   author={Chan, Ying-Hong and Fan, Yao-Chung},
%   booktitle={Proceedings of the 2nd workshop on machine reading for question answering},
%   pages={154--162},
%   year={2019}
% }

% @inproceedings{wang2022towards,
%   title={Towards human-like educational question generation with large language models},
%   author={Wang, Zichao and Valdez, Jakob and Basu Mallick, Debshila and Baraniuk, Richard G},
%   booktitle={International conference on artificial intelligence in education},
%   pages={153--166},
%   year={2022},
%   organization={Springer}
% }

[35], [44], [45], [46], [47] [48] [127] [128]
SolveMWPsunder zero/few-shotsetting

@article{lu2024chameleon,
  title={Chameleon: Plug-and-play compositional reasoning with large language models},
  author={Lu, Pan and Peng, Baolin and Cheng, Hao and Galley, Michel and Chang, Kai-Wei and Wu, Ying Nian and Zhu, Song-Chun and Gao, Jianfeng},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@article{wang2023plan,
  title={Plan-and-solve prompting: Improving zero-shot chain-of-thought reasoning by large language models},
  author={Wang, Lei and Xu, Wanyu and Lan, Yihuai and Hu, Zhiqiang and Lan, Yunshi and Lee, Roy Ka-Wei and Lim, Ee-Peng},
  journal={arXiv preprint arXiv:2305.04091},
  year={2023}
}

@article{zhang2022automatic,
  title={Automatic chain of thought prompting in large language models},
  author={Zhang, Zhuosheng and Zhang, Aston and Li, Mu and Smola, Alex},
  journal={arXiv preprint arXiv:2210.03493},
  year={2022}
}

@article{zhou2022least,
  title={Least-to-most prompting enables complex reasoning in large language models},
  author={Zhou, Denny and Sch{\"a}rli, Nathanael and Hou, Le and Wei, Jason and Scales, Nathan and Wang, Xuezhi and Schuurmans, Dale and Cui, Claire and Bousquet, Olivier and Le, Quoc and others},
  journal={arXiv preprint arXiv:2205.10625},
  year={2022}
}

@article{zheng2023progressive,
  title={Progressive-hint prompting improves reasoning in large language models},
  author={Zheng, Chuanyang and Liu, Zhengying and Xie, Enze and Li, Zhenguo and Li, Yu},
  journal={arXiv preprint arXiv:2304.09797},
  year={2023}
}

@article{chen2022program,
  title={Program of thoughts prompting: Disentangling computation from reasoning for numerical reasoning tasks},
  author={Chen, Wenhu and Ma, Xueguang and Wang, Xinyi and Cohen, William W},
  journal={arXiv preprint arXiv:2211.12588},
  year={2022}
}

@article{wei2022chain,
  title={Chain-of-thought prompting elicits reasoning in large language models},
  author={Wei, Jason and Wang, Xuezhi and Schuurmans, Dale and Bosma, Maarten and Xia, Fei and Chi, Ed and Le, Quoc V and Zhou, Denny and others},
  journal={Advances in neural information processing systems},
  volume={35},
  pages={24824--24837},
  year={2022}
}

@article{gou2023tora,
  title={Tora: A tool-integrated reasoning agent for mathematical problem solving},
  author={Gou, Zhibin and Shao, Zhihong and Gong, Yeyun and Yang, Yujiu and Huang, Minlie and Duan, Nan and Chen, Weizhu and others},
  journal={arXiv preprint arXiv:2309.17452},
  year={2023}
}

math \cite{lu2024chameleon,wang2023plan,zhang2022automatic,zhang2022automatic,zhou2022least,zheng2023progressive,chen2022program,wei2022chain,wei2022chain,gou2023tora}

\cite{lu2024chameleon}        &QS   & student & math          & K-12              & EN     & text & 8.5K   & \cite{cobbe2021training}\\
         
        \cite{wang2023plan} 

        \cite{zhang2022automatic}
        
        \cite{zhou2022least}

        \cite{zheng2023progressive}

        \cite{chen2022program}

        \cite{wei2022chain}

        \cite{gou2023tora}

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Strengthen zero-shot capabilities


@article{lu2022learn,
  title={Learn to explain: Multimodal reasoning via thought chains for science question answering},
  author={Lu, Pan and Mishra, Swaroop and Xia, Tanglin and Qiu, Liang and Chang, Kai-Wei and Zhu, Song-Chun and Tafjord, Oyvind and Clark, Peter and Kalyan, Ashwin},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={2507--2521},
  year={2022}
}

@inproceedings{chen2023theoremqa,
  title={Theoremqa: A theorem-driven question answering dataset},
  author={Chen, Wenhu and Yin, Ming and Ku, Max and Lu, Pan and Wan, Yixin and Ma, Xueguang and Xu, Jianyu and Wang, Xinyi and Xia, Tony},
  booktitle={The 2023 Conference on Empirical Methods in Natural Language Processing},
  year={2023}
}

@article{wang2023t,
  title={T-sciq: Teaching multimodal chain-of-thought reasoning via large language model signals for science question answering},
  author={Wang, Lei and Hu, Yi and He, Jiabang and Xu, Xing and Liu, Ning and Liu, Hui and Shen, Heng Tao},
  journal={arXiv preprint arXiv:2305.03453},
  year={2023}
}

@article{wang2023augmenting,
  title={Augmenting black-box llms with medical textbooks for clinical question answering},
  author={Wang, Yubo and Ma, Xueguang and Chen, Wenhu},
  journal={arXiv preprint arXiv:2309.02233},
  year={2023}
}

@article{liu2024visual,
  title={Visual instruction tuning},
  author={Liu, Haotian and Li, Chunyuan and Wu, Qingyang and Lee, Yong Jae},
  journal={Advances in neural information processing systems},
  volume={36},
  year={2024}
}

@article{lu2024chameleon,
  title={Chameleon: Plug-and-play compositional reasoning with large language models},
  author={Lu, Pan and Peng, Baolin and Cheng, Hao and Galley, Michel and Chang, Kai-Wei and Wu, Ying Nian and Zhu, Song-Chun and Gao, Jianfeng},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

\cite{lu2022learn,chen2023theoremqa,wang2023t,wang2023augmenting,liu2024visual,lu2024chameleon}
    \hline
         \cite{lu2022learn}        &QS   & student & math          & K-12              & EN     & text & 8.5K   & \cite{cobbe2021training}\\
         
        \cite{chen2023theoremqa} 

        \cite{wang2023t}
        
        \cite{wang2023augmenting}

        \cite{liu2024visual}

        \cite{lu2024chameleon}
test book      
[1] applied GPT-3 to solve the textbook question answering.
[2] introduced a system, that f irst retrieves the theories from the open domain and then answers the question based on the retrieved theories
[32] distilling the training signals from the LLMs to a smaller model
[33] augmented queries for LLMs on textbook question answering by retrieving evidences from textbooks, such that the response of the LLMs would likely to be authorized by the textbooks
[34] extended the instruction tuning to a multi-modal LLM
[35] develop compositional reasoning with LLMs as a planner that assembles a sequence of tools to execute and answer the textbook questions

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Identifyandcorrect grammarerrors accurately

Designmanualrulesandclassification-based models[91], [92];neuralnetworkmodelslike seq2seqmodels[93], [94], [95], [96], [97]and seq2editmodels[98], [99], [100], [101].



@article{fang2023chatgpt,
  title={Is chatgpt a highly fluent grammatical error correction system? a comprehensive evaluation},
  author={Fang, Tao and Yang, Shu and Lan, Kaixin and Wong, Derek F and Hu, Jinpeng and Chao, Lidia S and Zhang, Yue},
  journal={arXiv preprint arXiv:2304.01746},
  year={2023}
}

@article{alikaniotis2019under,
  title={Under the Hood at Grammarly: Leveraging Transformer Language Models for Grammatical Error Correction|},
  author={Alikaniotis, D and Raheja, V},
  journal={Grammarly Engineering Blog},
  year={2019}
}

@article{yasunaga2021lm,
  title={LM-critic: Language models for unsupervised grammatical error correction},
  author={Yasunaga, Michihiro and Leskovec, Jure and Liang, Percy},
  journal={arXiv preprint arXiv:2109.06822},
  year={2021}
}

@inproceedings{fan2023grammargpt,
  title={Grammargpt: Exploring open-source llms for native chinese grammatical error correction with supervised fine-tuning},
  author={Fan, Yaxin and Jiang, Feng and Li, Peifeng and Li, Haizhou},
  booktitle={CCF International Conference on Natural Language Processing and Chinese Computing},
  pages={69--80},
  year={2023},
  organization={Springer}
}

@article{li2023effectiveness,
  title={On the (in) effectiveness of large language models for chinese text correction},
  author={Li, Yinghui and Huang, Haojing and Ma, Shirong and Jiang, Yong and Li, Yangning and Zhou, Feng and Zheng, Hai-Tao and Zhou, Qingyu},
  journal={arXiv preprint arXiv:2307.09007},
  year={2023}
}

@inproceedings{yang2023let,
  title={LET: Leveraging Error Type Information for Grammatical Error Correction},
  author={Yang, Lingyu and Li, Hongjia and Li, Lei and Xu, Chengyin and Xia, Shutao and Yuan, Chun},
  booktitle={Findings of the Association for Computational Linguistics: ACL 2023},
  pages={5986--5998},
  year={2023}
}

@article{kwon2023beyond,
  title={Beyond English: Evaluating LLMs for Arabic Grammatical Error Correction},
  author={Kwon, Sang Yun and Bhatia, Gagan and Nagoudi, El Moatez Billah and Abdul-Mageed, Muhammad},
  journal={arXiv preprint arXiv:2312.08400},
  year={2023}
}

@article{li2024rethinking,
  title={Rethinking the Roles of Large Language Models in Chinese Grammatical Error Correction},
  author={Li, Yinghui and Qin, Shang and Ye, Jingheng and Ma, Shirong and Li, Yangning and Qin, Libo and Hu, Xuming and Jiang, Wenhao and Zheng, Hai-Tao and Yu, Philip S},
  journal={arXiv preprint arXiv:2402.11420},
  year={2024}
}

\cite{fang2023chatgpt,alikaniotis2019under,yasunaga2021lm,fan2023grammargpt,li2023effectiveness,yang2023let,kwon2023beyond,li2024rethinking}

\cite{fang2023chatgpt}

\cite{alikaniotis2019under}

\cite{yasunaga2021lm}

\cite{fan2023grammargpt}

\cite{li2023effectiveness}

\cite{yang2023let}

\cite{kwon2023beyond}

\cite{li2024rethinking}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Identifyandcorrect errorsinthelongdistancedependency of thecode


@article{chen2023teaching,
  title={Teaching large language models to self-debug},
  author={Chen, Xinyun and Lin, Maxwell and Sch{\"a}rli, Nathanael and Zhou, Denny},
  journal={arXiv preprint arXiv:2304.05128},
  year={2023}
}

@article{cao2023study,
  title={A study on prompt design, advantages and limitations of chatgpt for deep learning program repair},
  author={Cao, Jialun and Li, Meiziniu and Wen, Ming and Cheung, Shing-chi},
  journal={arXiv preprint arXiv:2304.08191},
  year={2023}
}

@inproceedings{mahbub2023explaining,
  title={Explaining software bugs leveraging code structures in neural machine translation},
  author={Mahbub, Parvez and Shuvo, Ohiduzzaman and Rahman, Mohammad Masudur},
  booktitle={2023 IEEE/ACM 45th International Conference on Software Engineering (ICSE)},
  pages={640--652},
  year={2023},
  organization={IEEE}
}


@article{pan2023understanding,
  title={Understanding the effectiveness of large language models in code translation},
  author={Pan, Rangeet and Ibrahimzada, Ali Reza and Krishna, Rahul and Sankar, Divya and Wassi, Lambert Pouguem and Merler, Michele and Sobolev, Boris and Pavuluri, Raju and Sinha, Saurabh and Jabbarvand, Reyhaneh},
  journal={arXiv preprint arXiv:2308.03109},
  year={2023}
}

@article{bui2022detect,
  title={Detect-localize-repair: A unified framework for learning to debug with codet5},
  author={Bui, Nghi DQ and Wang, Yue and Hoi, Steven},
  journal={arXiv preprint arXiv:2211.14875},
  year={2022}
}

@inproceedings{kang2023large,
  title={Large language models are few-shot testers: Exploring llm-based general bug reproduction},
  author={Kang, Sungmin and Yoon, Juyeon and Yoo, Shin},
  booktitle={2023 IEEE/ACM 45th International Conference on Software Engineering (ICSE)},
  pages={2312--2323},
  year={2023},
  organization={IEEE}
}

@article{kang2023preliminary,
  title={A preliminary evaluation of llm-based fault localization},
  author={Kang, Sungmin and An, Gabin and Yoo, Shin},
  journal={arXiv preprint arXiv:2308.05487},
  year={2023}
}

@article{widjojo2023addressing,
  title={Addressing compiler errors: Stack overflow or large language models?},
  author={Widjojo, Patricia and Treude, Christoph},
  journal={arXiv preprint arXiv:2307.10793},
  year={2023}
}

@article{plein2023can,
  title={Can llms demystify bug reports?},
  author={Plein, Laura and Bissyand{\'e}, Tegawend{\'e} F},
  journal={arXiv preprint arXiv:2310.06310},
  year={2023}
}

@inproceedings{taylor2023dcc,
  title={Dcc-help: Generating context-aware compiler error explanations with large language models},
  author={Taylor, Andrew and Vassar, Alexandra and Renzella, Jake and Pearce, Hammond},
  booktitle={Proceedings of the 55 th ACM Technical Symp. on Computer Science Education},
  volume={1},
  year={2023}
}

@article{kang2023explainable,
  title={Explainable automated debugging via large language model-driven scientific debugging},
  author={Kang, Sungmin and Chen, Bei and Yoo, Shin and Lou, Jian-Guang},
  journal={arXiv preprint arXiv:2304.02195},
  year={2023}
}

@inproceedings{yang2024large,
  title={Large language models for test-free fault localization},
  author={Yang, Aidan ZH and Le Goues, Claire and Martins, Ruben and Hellendoorn, Vincent},
  booktitle={Proceedings of the 46th IEEE/ACM International Conference on Software Engineering},
  pages={1--12},
  year={2024}
}

@article{tu2023llm4cbi,
  title={LLM4CBI: taming llms to generate effective test programs for compiler bug isolation},
  author={Tu, Haoxin and Zhou, Zhide and Jiang, He and Yusuf, Imam Nur Bani and Li, Yuxian and Jiang, Lingxiao},
  journal={arXiv preprint arXiv:2307.00593},
  year={2023}
}

@inproceedings{li2023nuances,
  title={Nuances are the key: Unlocking chatgpt to find failure-inducing tests with differential prompting},
  author={Li, Tsz-On and Zong, Wenxi and Wang, Yibo and Tian, Haoye and Wang, Ying and Cheung, Shing-Chi and Kramer, Jeff},
  booktitle={2023 38th IEEE/ACM International Conference on Automated Software Engineering (ASE)},
  pages={14--26},
  year={2023},
  organization={IEEE}
}


\cite{chen2023teaching,cao2023study,mahbub2023explaining,pan2023understanding,bui2022detect,kang2023large,kang2023preliminary,widjojo2023addressing,plein2023can,taylor2023dcc,kang2023explainable,yang2024large,tu2023llm4cbi,li2023nuances}

\cite{chen2023teaching}

\cite{cao2023study}

\cite{mahbub2023explaining}

\cite{pan2023understanding}

\cite{bui2022detect}

\cite{kang2023large}

\cite{kang2023preliminary}

\cite{widjojo2023addressing}

\cite{plein2023can}

\cite{taylor2023dcc}

\cite{kang2023explainable}

\cite{yang2024large}

\cite{tu2023llm4cbi}

\cite{li2023nuances}




c (in EMNLP 2022)
Large Language Models are Few-shot Testers: Exploring LLM-based General Bug Reproduction (in ICSE 2023)
A Preliminary Evaluation of LLM-Based Fault Localization (in Arxiv)
Addressing Compiler Errors: Stack Overflow or Large Language Models? (in Arxiv)
Can LLMs Demystify Bug Reports? (in Arxiv)
Dcc --help: Generating Context-Aware Compiler Error Explanations with Large Language Models (in SIGCSE 2024)
Explainable Automated Debugging via Large Language Model-driven Scientific Debugging (in Arxiv)
Large Language Models for Test-Free Fault Localization (in ICSE 2024)
Large Language Models in Fault Localisation (in Arxiv)
LLM4CBI: Taming LLMs to Generate Effective Test Programs for Compiler Bug Isolation (in Arxiv)
Nuances are the Key: Unlocking ChatGPT to Find Failure-Inducing Tests with Differential Prompting (in ASE 2023)
Teaching Large Language Models to Self-Debug (in Arxiv)
A study on Prompt Design, Advantages and Limitations of ChatGPT for Deep Learning Program Repair (in Arxiv)



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With the advent of languagemodels, theBERT modelandLLMGPT-3havebeenappliedtoQG[142],[143]. Besides, regardinganswer informationintheQGsystem, researchersproposedtoencode theanswer togetherwith the context [144], utilize theposition informationof the answerinthecontext[145],[146],andachieveanswer-aware QG,whileusingsummariesof thetextsasinputcanserve as a strategy for answer-agnosticQGas it canhelp the modelingof topicsalience,whichdenotes the importance ofspecificwordsorphrasesincontext[130].

\cite{chan2019recurrent,wang2022towards,yuan2017machine,sun2018answer,ma2020improving}

@inproceedings{chan2019recurrent,
  title={A recurrent BERT-based model for question generation},
  author={Chan, Ying-Hong and Fan, Yao-Chung},
  booktitle={Proceedings of the 2nd workshop on machine reading for question answering},
  pages={154--162},
  year={2019}
}

@inproceedings{wang2022towards,
  title={Towards human-like educational question generation with large language models},
  author={Wang, Zichao and Valdez, Jakob and Basu Mallick, Debshila and Baraniuk, Richard G},
  booktitle={International conference on artificial intelligence in education},
  pages={153--166},
  year={2022},
  organization={Springer}
}

@article{yuan2017machine,
  title={Machine comprehension by text-to-text neural question generation},
  author={Yuan, Xingdi and Wang, Tong and Gulcehre, Caglar and Sordoni, Alessandro and Bachman, Philip and Subramanian, Sandeep and Zhang, Saizheng and Trischler, Adam},
  journal={arXiv preprint arXiv:1705.02012},
  year={2017}
}

@inproceedings{sun2018answer,
  title={Answer-focused and position-aware neural question generation},
  author={Sun, Xingwu and Liu, Jing and Lyu, Yajuan and He, Wei and Ma, Yanjun and Wang, Shi},
  booktitle={Proceedings of the 2018 conference on empirical methods in natural language processing},
  pages={3930--3939},
  year={2018}
}

@inproceedings{ma2020improving,
  title={Improving question generation with sentence-level semantic matching and answer position inferring},
  author={Ma, Xiyao and Zhu, Qile and Zhou, Yanlin and Li, Xiaolin},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={34},
  number={05},
  pages={8464--8471},
  year={2020}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Developlanguagemodeling[102], [103];methods withabstractsyntaxtree[104], [105];denoising strategies[106];useidentifiertaggingandcomment information[107];grammarconstraints[108].


Generate more flexiblequestionsfor adaptiveeducation


generation-basedmethods[66], [67];

Designvariousfeatures(e.g. length-basedfeatures[71]; lexical features[71], [72];promptrelevant features[73]; readabilityfeatures[71]; syntacticfeatures[71], [74])andsolveviaregressionandranking[75]withenhancedtraining procedure[76].





%%%%%%%%%%%%%%%%%%%%%%%%%%%%




Decouplethedomain-dependentanddomainindependent featuresandaggregateheuristic supervisionsignals[77], [78], [79];designenriched annotations[80], [81].

    \hline
    \end{tabular}
    \caption{Summary of existing  dataset and benchmark in the area of education}
    \label{tab:dataset}
\end{table*}

\cite{gonzalez2021artificial,nicula2023automated,ormerod2021automated,gupta2023data,oli2023automated}

@article{gonzalez2021artificial,
  title={Artificial intelligence for student assessment: A systematic review},
  author={Gonz{\'a}lez-Calatayud, V{\'\i}ctor and Prendes-Espinosa, Paz and Roig-Vila, Rosabel},
  journal={Applied Sciences},
  volume={11},
  number={12},
  pages={5467},
  year={2021},
  publisher={MDPI}
}

@article{nicula2023automated,
  title={Automated Assessment of Comprehension Strategies from Self-Explanations Using LLMs},
  author={Nicula, Bogdan and Dascalu, Mihai and Arner, Tracy and Balyan, Renu and McNamara, Danielle S},
  journal={Information},
  volume={14},
  number={10},
  pages={567},
  year={2023},
  publisher={MDPI}
}

@article{ormerod2021automated,
  title={Automated essay scoring using efficient transformer-based language models},
  author={Ormerod, Christopher M and Malhotra, Akanksha and Jafari, Amir},
  journal={arXiv preprint arXiv:2102.13136},
  year={2021}
}

@inproceedings{gupta2023data,
  title={Data Augmentation for Automated Essay Scoring using Transformer Models},
  author={Gupta, Kshitij},
  booktitle={2023 International Conference on Artificial Intelligence and Smart Communication (AISC)},
  pages={853--857},
  year={2023},
  organization={IEEE}
}

@article{oli2023automated,
  title={Automated Assessment of Students' Code Comprehension using LLMs},
  author={Oli, Priti and Banjade, Rabin and Chapagain, Jeevan and Rus, Vasile},
  journal={arXiv preprint arXiv:2401.05399},
  year={2023}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


https://learn.microsoft.com/en-us/training/modules/enhance-teaching-learning-bing-chat/

@misc{Microsoft2023EnhanceTeaching,
  title = {Enhance Teaching and Learning with Bing Chat},
  organization = {Microsoft},
  url = {https://learn.microsoft.com/en-us/training/modules/enhance-teaching-learning-bing-chat/},
  %note = {Accessed: [your access date here]}
}




        %     forked edges,
            % for tree={
            %     fill=level0!80,
            %     grow=east,
            %     reversed=true,
            %     anchor=base west,
            %     parent anchor=east,
            %     child anchor=west,
            %     base=left,
            %     font=\large,
            %     rectangle,
            %     draw=hidden-draw,
            %     rounded corners,
            %     align=left,
            %     minimum width=4em,
            %     edge+={darkgray, line width=1pt},
            %     s sep=3pt,
            %     inner xsep=2pt,
            %     inner ysep=3pt,
            %     line width=0.8pt,
            %     ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            % },
            % where level=1{text width=8em,font=\normalsize,fill=level1!80,}{},
            % where level=2{text width=9.5em,font=\normalsize,fill=level2!80,}{},
            % where level=3{text width=11.5em,font=\normalsize,fill=level3!60,}{},
            % where level=4{text width=10em,font=\normalsize,fill=level4!20,}{},
            % where level=5{text width=5em,font=\normalsize,}{},
            % [
            %     Large Language Models \\ in Education 
            %     [Academic \\Researches
            %     [
            %         Study Assisting
            %         [
            %            Question Solving (QS)
            %                         [ 
            %                             Math \cite{yuan2023well,wu2023empirical,sun2023offline,wang2023large,lu2024chameleon,wang2023plan,zhang2022automatic,zhang2022automatic,zhou2022least,zheng2023progressive,chen2022program,wei2022chain,wei2022chain,gou2023tora}\\
            %                             Science \cite{lu2022learn,chen2023theoremqa,wang2023t,wang2023augmenting,liu2024visual,lu2024chameleon}
            %                             Law \cite{bommarito2022gpt,cui2023chatlaw} \\
            %                             Medicine \cite{thirunavukarasu2023large,lievin2023can} \\ 
            %                             Finance \cite{wu2023bloomberggpt,yang2023fingpt} \\
            %                             Programming \cite{kazemitabaar2023novices,savelka2023thrilled} \\
            %                             Language Understands \cite{zhang2024m3exam,achiam2023gpt}, leaf, text width=32em
            %                         ]
            %         ]
            %         [
            %            Error Correction (EC)
            %                         [ 
            %                             Grammar Error Correction~\cite{fang2023chatgpt,alikaniotis2019under,yasunaga2021lm,fan2023grammargpt,li2023effectiveness,yang2023let,kwon2023beyond,li2024rethinking}\\
            %                             Program Bug Repair~\cite{chen2023teaching,cao2023study,mahbub2023explaining,pan2023understanding,bui2022detect,kang2023large,kang2023preliminary,widjojo2023addressing,plein2023can,taylor2023dcc,kang2023explainable,yang2024large,tu2023llm4cbi,li2023nuances}, leaf, text width=32em
            %                         ]
            %         ]
            %         [
            %            Confusion Helper (CH)
            %                         [ 
            %                             Explain and Hint Generation~\cite{shridharautomatic,prihar2023comparing,pardos2023learning,balse2023evaluating,rooein2023know}, leaf, text width=32em
            %                         ]
            %         ]
            %     ]

            %     [
            %         Teach Assisting
            %         [
            %            Question Generation (QG)
            %                         [ 
            %                             Reading Comprehension~\cite{chan2019recurrent,wang2022towards,yuan2017machine,sun2018answer,ma2020improving,xiao2023evaluating,lee2023few}\\
            %                             Computer Programming~\cite{doughty2024comparative}\\
            %                             Math Word Problem~\cite{zhou2023learning,christ2024mathwell,norberg2023rewriting,liang2023let},leaf, text width=32em
            %                         ]
            %         ]
            %         [
            %            Automatic Grading (AG)
            %                         [ 
            %                             Writing Essay~\cite{gonzalez2021artificial,nicula2023automated,ormerod2021automated,gupta2023data,oli2023automated,pinto2023large,xiao2024automation}\\
            %                             Math Answers~\cite{urrutia2024s,li2024automated}\\
            %                             Short Textual Answers~\cite{schneider2023towards,kortemeyer2023performance,morjaria2024examining,henkel2023can}, leaf, text width=32em
            %                         ]
            %         ]
            %         [
            %            Material Creation (MC)
            %                         [ 
            %                             Course Content~\cite{leiker2023prototyping,koraishi2023teaching} \\ 
            %                             Illustration Examples~\cite{jury2024evaluating}, leaf, text width=32em
            %                         ]
            %         ]
            %     ]

            %     [
            %         Adaptive Learning
            %         [
            %            Knowledge Tracing (KT)
            %                         [ 
            %                             KT Data Enhancing~\cite{ni2023enhancing,lee2023difficulty} \\Student Behaviour Simulation~\cite{sonkar2023deduction,liu2022gpt}, leaf, text width=32em
            %                         ]
            %         ]
            %         [
            %            Content Personalizing (CP)
            %                         [ 
            %                             Learning Path~\cite{kuo2023leveraging,kabir2023llm} \\
            %                             Question and Explanation ~\cite{yadav2023contextualizing,abu2024knowledge}, leaf, text width=32em
            %                         ]
            %         ]
            %     ]
            %     ]

            %     [
            %         Commercial Tools
            %         [
            %            Chatbot \cite{Microsoft2023EnhanceTeaching,OpenAIChat,PerplexityAI,GoogleBard,PiAI}, leaf, text width=23em
            %         ]
            %         [
            %            Content Creation \cite{Curipod,Diffit,MagicSchoolAI,Education_Copilot,Nolej,Eduaide_ai,Khanmigo,Copy_ai}, leaf, text width=23em
            %         ]
            %         [
            %            Teaching Aide \cite{gotFeedbackbygotLearning,Grammarly,Goblin_Tools,Chat_PDF}, leaf, text width=23em
            %         ]
            %         [
            %            Quiz Generator \cite{QuestionWell,Formative_AI,Quizizz_AI,Conker,Twee}, leaf, text width=23em
            %         ]
            %         [
            %            Collaboration Tool \cite{summarize_tech,Parlay_Genie}, leaf, text width=23em
            %         ]                
            %     ]
            % ]




            \tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left, font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[!t]
    \centering
    \resizebox{0.85\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                fill=level0!80,
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=8em,font=\normalsize,fill=level1!80,}{},
            where level=2{text width=9.5em,font=\normalsize,fill=level2!80,}{},
            where level=3{text width=11.5em,font=\normalsize,fill=level3!60,}{},
            where level=4{text width=10em,font=\normalsize,fill=level4!20,}{},
            where level=5{text width=5em,font=\normalsize,}{},
            [
                Large Language Models \\ in Education 
                [Academic \\Researches
                [
                    Study Assisting
                    [
                       Question Solving (QS)
                                    [ 
                                        Math \cite{yuan2023well,wu2023empirical,sun2023offline,wang2023large,lu2024chameleon,wang2023plan,zhang2022automatic,zhang2022automatic,zhou2022least,zheng2023progressive,chen2022program,wei2022chain,wei2022chain,gou2023tora}\\
                                        Science \cite{lu2022learn,chen2023theoremqa,wang2023t,wang2023augmenting,liu2024visual,lu2024chameleon}
                                        Law \cite{bommarito2022gpt,cui2023chatlaw} \\
                                        Medicine \cite{thirunavukarasu2023large,lievin2023can} \\ 
                                        Finance \cite{wu2023bloomberggpt,yang2023fingpt} \\
                                        Programming \cite{kazemitabaar2023novices,savelka2023thrilled} \\
                                        Language Understands \cite{zhang2024m3exam,achiam2023gpt}, leaf, text width=32em
                                    ]
                    ]
                    [
                       Error Correction (EC)
                                    [ 
                                        Grammar Error Correction~\cite{fang2023chatgpt,alikaniotis2019under,yasunaga2021lm,fan2023grammargpt,li2023effectiveness,yang2023let,kwon2023beyond,li2024rethinking}
 \\
                                        Program Bug Repair~\cite{chen2023teaching,cao2023study,mahbub2023explaining,pan2023understanding,bui2022detect,kang2023large,kang2023preliminary,widjojo2023addressing,plein2023can,taylor2023dcc,kang2023explainable,yang2024large,tu2023llm4cbi,li2023nuances}, leaf, text width=32em
                                    ]
                    ]
                    [
                       Confusion Helper (CH)
                                    [ 
                                        Explain and Hint Generation~\cite{shridharautomatic,prihar2023comparing,pardos2023learning,balse2023evaluating,rooein2023know}, leaf, text width=32em
                                    ]
                    ]
                ]

                [
                    Teach Assisting
                    [
                       Question Generation (QG)
                                    [ 
                                        Reading Comprehension~\cite{chan2019recurrent,wang2022towards,yuan2017machine,sun2018answer,ma2020improving,xiao2023evaluating,lee2023few}\\
                                        Computer Programming~\cite{doughty2024comparative}\\
                                        Math Word Problem~\cite{zhou2023learning,christ2024mathwell,norberg2023rewriting,liang2023let},leaf, text width=32em
                                    ]
                    ]
                    [
                       Automatic Grading (AG)
                                    [ 
                                        Writing Essay~\cite{gonzalez2021artificial,nicula2023automated,ormerod2021automated,gupta2023data,oli2023automated,pinto2023large,xiao2024automation}\\
                                        Math Answers~\cite{urrutia2024s,li2024automated}\\
                                        Short Textual Answers~\cite{schneider2023towards,kortemeyer2023performance,morjaria2024examining,henkel2023can}, leaf, text width=32em
                                    ]
                    ]
                    [
                       Material Creation (MC)
                                    [ 
                                        Course Content~\cite{leiker2023prototyping,koraishi2023teaching} \\ 
                                        Illustration Examples~\cite{jury2024evaluating}, leaf, text width=32em
                                    ]
                    ]
                ]

                [
                    Adaptive Learning
                    [
                       Knowledge Tracing (KT)
                                    [ 
                                        KT Data Enhancing~\cite{ni2023enhancing,lee2023difficulty} \\Student Behaviour Simulation~\cite{sonkar2023deduction,liu2022gpt}, leaf, text width=32em
                                    ]
                    ]
                    [
                       Content Personalizing (CP)
                                    [ 
                                        Learning Path~\cite{kuo2023leveraging,kabir2023llm} \\
                                        Question and Explanation ~\cite{yadav2023contextualizing,abu2024knowledge}, leaf, text width=32em
                                    ]
                    ]
                ]
                ]

                [
                    Commercial Tools
                    [
                       Chatbot \cite{Microsoft2023EnhanceTeaching,OpenAIChat,PerplexityAI,GoogleBard,PiAI}, leaf, text width=23em
                    ]
                    [
                       Content Creation \cite{Curipod,Diffit,MagicSchoolAI,Education_Copilot,Nolej,Eduaide_ai,Khanmigo,Copy_ai}, leaf, text width=23em
                    ]
                    [
                       Teaching Aide \cite{gotFeedbackbygotLearning,Grammarly,Goblin_Tools,Chat_PDF}, leaf, text width=23em
                    ]
                    [
                       Quiz Generator \cite{QuestionWell,Formative_AI,Quizizz_AI,Conker,Twee}, leaf, text width=23em
                    ]
                    [
                       Collaboration Tool \cite{summarize_tech,Parlay_Genie}, leaf, text width=23em
                    ]                
                ]
            ]
        \end{forest}
    }\vspace{-3mm}
\caption{A taxonomy of LLMs for education applications with representative works.} \vspace{-4mm}
\label{fig:taxonomy}
\end{figure*}
